Post-Newtonian Gravity in Cosmology

The post-Newtonian (PN) perturbative framework has been successful in understanding the slow-motion, weak field limit of Einstein's theory of gravity on solar system scales, and for isolated astrophysical systems. The parameterized post-Newtonian (PPN) formalism extended the PN framework to put very tight constraints on deviations from Einstein's theory on the aforementioned scales and systems. In this work, we extended and applied the post-Newtonian formalism to cosmological scales. We first used it to construct a cosmological model to understand the effect of regularly arranged point sources on the background expansion. Here we found that at higher orders we obtained a small radiation-like correction to the standard Friedmann-Lema\^{i}tre-Robertson-Walker (FLRW) equations, for a matter-dominated universe. This radiation-like correction was purely due to the inhomogeneity of our model, and the non-linearity of Einstein's field equations. We also extended the post-Newtonian formalism to include other forms of matter that are cosmologically relevant, such as radiation and a cosmological constant, and studied the non-linear effects they might have on the background expansion. Then we constructed an extension of the parameterized post-Newtonian formalism (PPN) to cosmological scales. We used it to parameterize the background expansion of the universe as well as first-order perturbations in cosmology, using four functions of time. We gave examples of how our parameterization would work for dark energy models and scalar-tensor and vector-tensor theories of gravity. In the final part of this work, we studied how light propagation behaves in an inhomogeneous post-Newtonian cosmology with matter and a cosmological constant. We used it to understand the effect that inhomogeneities would have on observables.

==> macros.tex <==
% Abréviations maths

\newcommand\ph{\ensuremath{\varphi}}
\newcommand\eps{\ensuremath{\varepsilon}}

\newcommand{\cc}{\text{c.c.}}
\newcommand{\cst}{\mathrm{cst}}
\newcommand{\sgn}{\mathrm{sgn}}

%\newcommand\define{\overset{\text{déf.}}{=}}
\newcommand\define{\equiv}
\newcommand{\coordequal}{\overset{*}{=}}
\newcommand\alg[1]{\overline{#1}}
%\newcommand\vect[1]{\overrightarrow{#1}}
\newcommand\vect[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\newcommand\cplx[1]{\underline{#1}}
\newcommand\ex[1]{\mathrm{e}^{#1}}
\renewcommand\i{\ensuremath{\mathrm{i}}}
\renewcommand\j{\ensuremath{\mathrm{j}}}
\renewcommand\Re{\ensuremath{\mathrm{Re}}}
\renewcommand\Im{\ensuremath{\mathrm{Im}}}
\newcommand{\Arg}{\ensuremath{\mathrm{Arg}}}
\newcommand\suite[3]{\ensuremath{(#1)_{#2\in{#3}}}}
\newcommand\transpose[1]{#1^{\rm T}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand\colonne[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand\gcolonne[2]{\begin{pmatrix} #1 \\[1mm] #2 \end{pmatrix}}
\newcommand\Ker{\mathrm{Ker}}

\newcommand\e[1]{_{\text{#1}}}
\newcommand\h[1]{^{\text{#1}}}
\newcommand\U[1]{\:\mathrm{#1}}
\newcommand{\micro}{\hbox{\textmu}}

\newcommand{\dd}{\mathrm{d}}
\newcommand{\Dd}{\mathrm{D}}
\newcommand{\pd}[3][]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}
\newcommand{\ddf}[3][]{\frac{\dd^{#1} #2}{\dd {#3}^{#1}}}
\newcommand{\Ddf}[3][]{\frac{\Dd^{#1} #2}{\dd {#3}^{#1}}}

\newcommand{\grad}{\vect{\nabla}}

%\renewcommand\lim[2]{\underset{ #1 \rightarrow #2 }{ \mathrm{lim} } \,}
\newcommand\tendvers[2]{\underset{#1 \rightarrow #2}{\longrightarrow}}

\newcommand{\delimiters}[4][]{
\ifthenelse{ \equal{#1}{1} }{  #2 #3 #4  }
					{ \ifthenelse{\equal{#1}{2}}{ \big#2 #3 \big#4 }
						{ \ifthenelse{\equal{#1}{3}}{ \Big#2 #3 \Big#4 }
							{ \ifthenelse{\equal{#1}{4}}{ \bigg#2 #3 \bigg#4 }
								{ \ifthenelse{\equal{#1}{5}}{ \Bigg#2 #3 \Bigg#4 }
									{ \left#2 #3 \right#4 }
								}
							}
						}
					}
													}

\newcommand{\pa}[2][]{\delimiters[#1]{(}{#2}{)}}
\newcommand{\pac}[2][]{\delimiters[#1]{[}{#2}{]}}
\newcommand{\paac}[2][]{\delimiters[#1]{\{}{#2}{\}}}
\newcommand{\abs}[2][]{\delimiters[#1]{|}{#2}{|}}
\newcommand{\ev}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\evaluate}[2][]{\delimiters[#1]{.}{#2}{|}}
\newcommand{\mean}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\ket}[2][]{\delimiters[#1]{|}{#2}{\rangle}}
\newcommand{\bra}[2][]{\delimiters[#1]{\langle}{#2}{|}}

\newcommand{\source}{\mathrm{s}}
\newcommand{\obs}{\mathrm{o}}
\newcommand{\PF}[1]{\textcolor{red}{#1}}
\newcommand{\varDA}{\sigma_{D\e{A}}^2}

\newcommand{\tidal}{\mathcal{R}}
\newcommand{\jacobi}{\mathcal{D}}
\newcommand{\wronski}{\mathcal{W}}
\newcommand{\amplification}{\mathcal{A}}
\newcommand{\deformation}{\mathcal{S}}
\newcommand{\Ricfoc}{\mathscr{R}}
\newcommand{\Weylfoc}{\mathscr{W}}

\newcommand{\Lie}{\mathcal{L}}
\newcommand{\wl}{\mathscr{L}}

\newcommand{\Hc}{\mathcal{H}}

\newcommand{\nul}[1]{%\hat{#1}
#1}

\newcommand{\zero}{\mat{0}}
\newcommand{\identity}{\mat{1}}


\newenvironment{system}
{ \left\{ \begin{aligned} }
{ \end{aligned} \right. }

\newenvironment{remark}
{

\medskip

\noindent
\hspace{0.05\linewidth}
\vline
\hspace{0.01\linewidth}
\begin{minipage}{0.93\linewidth}
}
{
\end{minipage}

\medskip

}

% Box
\newlength{\boxtitlelength}
\newlength{\halfrulelength}
\newcommand{\boxtitle}[1]{\footnotesize\bf{\:#1\:}}
\newenvironment{abox}[1]
{
\setlength{\halfrulelength}{0.5\linewidth}
\settowidth{\boxtitlelength}{\boxtitle{#1}}
\addtolength{\halfrulelength}{-0.5\boxtitlelength}
\noindent\rule[-1mm+1pt]{1pt}{2mm}\rule[1mm]{\halfrulelength}{1pt}{\boxtitle{#1}}\rule[1mm]{\halfrulelength}{1pt}\rule[-1mm+1pt]{1pt}{2mm}\\}
{\\ \rule[1mm]{1pt}{2mm}\noindent\rule[1mm]{\linewidth-2pt}{1pt}\rule[1mm]{1pt}{2mm}}

% Create a command for sections hidden in the text
\newcommand{\hiddensection}[1]{
\refstepcounter{section}
\phantomsection
\addcontentsline{toc}{section}{\protect\numberline{\thesection}#1}
\markright{\thesection \: #1}
}

% Colors

\definecolor{blue4}{RGB}{0,0,143}
\definecolor{red4}{RGB}{143,0,0}
\definecolor{orange}{RGB}{255,128,0}
\definecolor{darkcyan}{RGB}{0,128,128}
\definecolor{olive}{RGB}{0,128,0}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{cyan2}{RGB}{0,255,255}
\definecolor{fushia}{RGB}{255,0,255}
\definecolor{mygray}{gray}{0.5}
\definecolor{lightgray}{gray}{0.85}

% Journals

\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjl}{ApJL}
\newcommand{\aap}{A{\&}A}
\newcommand{\aaps}{A{\&}AS}
\newcommand{\mnras}{MNRAS}
\newcommand{\aj}{AJ}
\newcommand{\araa}{ARAA}
\newcommand{\pasp}{PASP}
\newcommand{\pasj}{PASJ}
\newcommand{\jcap}{JCAP}
\newcommand{\na}{New Astronomy}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\azh}{Astron. Zh.}
\newcommand{\nat}{Nature}
\newcommand{\nar}{New Astronomy Reviews}


==> packages.tex <==
\usepackage{jcappub}
\usepackage{mathrsfs}
\usepackage{bbm}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{tensor}
\usepackage{xspace}
\usepackage{aeguill}
\usepackage{wasysym}
\usepackage{microtype}
\usepackage{empheq}
\usepackage{ifthen}
%\usepackage{subcaption}
\usepackage{amsmath}
%\usepackage[titletoc]{appendix}
%\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{wrapfig}

%\usepackage[frenchb,spanish,english]{babel}
%%\frenchbsetup{ReduceListSpacing=false}
%%\frenchbsetup{CompactItemize=false}
%%\frenchbsetup{StandardItemLabels=true}
%%\DecimalMathComma
%
%\usepackage[utf8x]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{ucs}
%\usepackage{textcomp}
%\usepackage{microtype}
%\usepackage{lmodern}
%
%\usepackage[small,labelfont={sf,bf},labelsep=quad]{caption}
%\usepackage{geometry}
%\usepackage{fancyhdr}
%\usepackage{fancybox}
%\usepackage{url}
%%\usepackage[pdfpagelabels,plainpages=false,urlcolor=blue]{hyperref}
%\usepackage{hyperref}
%%\usepackage{natbib}
%\usepackage{cite}
%%\usepackage{coverpages}
%%\usepackage{enumerate}
%
%\usepackage{xspace}
%\usepackage{lastpage}
%\usepackage{stmaryrd}
%
%\usepackage{graphicx}
%%\usepackage{subfigure}
%\usepackage{subcaption}
%%\usepackage[outercaption]{sidecap}
%%\usepackage{psfrag}
%\usepackage[table]{xcolor}
%\usepackage{rotating}
%\usepackage{empheq}
%\usepackage{ifthen}
%\usepackage{tensor}
%\usepackage{paralist}
%\usepackage{wrapfig}
%\usepackage{array}
%
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}
%\usepackage{mathrsfs}
%\usepackage{extarrows}
%\usepackage{verbatim}
%\usepackage{siunitx}
%\usepackage{upgreek}
%\usepackage{multirow}
%\usepackage[overload]{abraces} % des accolades horizontales plus élégantes
%
%\usepackage{makeidx}
%\usepackage[sectionbib]{chapterbib}
%
%\usepackage{lettrine}
%\usepackage{minitoc}
%%\usepackage[section]{placeins}
%
%\usepackage{pdfpages}
%%\usepackage[sf,bf,newlinetospace]{titlesec}
%%\usepackage{titletoc}
%%\titleformat{\subsubsection}{display}

